Fair Clustering Under a Bounded Cost

Clustering is a fundamental unsupervised learning problem where a dataset is partitioned into clusters that consist of nearby points in a metric space. A recent variant, fair clustering, associates a color with each point representing its group membership and requires that each color has (approximately) equal representation in each cluster to satisfy group fairness. In this model, the cost of the clustering objective increases due to enforcing fairness in the algorithm. The relative increase in the cost, the ''price of fairness,'' can indeed be unbounded. Therefore, in this paper we propose to treat an upper bound on the clustering objective as a constraint on the clustering problem, and to maximize equality of representation subject to it. We consider two fairness objectives: the group utilitarian objective and the group egalitarian objective, as well as the group leximin objective which generalizes the group egalitarian objective. We derive fundamental lower bounds on the approximation of the utilitarian and egalitarian objectives and introduce algorithms with provable guarantees for them. For the leximin objective we introduce an effective heuristic algorithm. We further derive impossibility results for other natural fairness objectives. We conclude with experimental results on real-world datasets that demonstrate the validity of our algorithms.

==> acknowledgments.tex <==
%\section*{Acknowledgments}
\noindent\textbf{Acknowledgments}


==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Our guarantees are free of assumptions. However, there is the issue of the dependence on the size of the smallest cluster at a given cost. This is discussed in detail and verified experimentally in Sections (\ref{sec:hardness},\ref{sec:algorithms}, \ref{lb_assump_exp}) and in Appendix \ref{lower_bound_appendix}. }
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Please see the appendix for the proofs.} 
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{The experiments do not involve training or tuning hyperparameters and the like.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{ We mention the hardware details in the paper and further note that it is commodity hardware that does not involve using GPUs.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

\clearpage 

==> constraint_set_squish.tex <==
\begin{subequations}\label{lpf}
  \begin{align}
     \sum_{i,j} d^p(i,j) x_{ij} \leq \upofp      \label{lpf_1} \\
    
    \forall j \in \Points: \sum_{i \in S} x_{ij}=1, \quad x_{ij} \in [0,1] \label{lpf_11} \\
    
    \forall h \in \Colors: \dpc \in [0,1] \label{lpf_dpc_orig} \\
   
    \forall \pcolor \in \Colors, \forall i \in S: 
    (\beta_h-\dpc) \Big( \sum_{j \in \Points} x_{ij} \Big) 
    \leq \sum_{j \in \Points^{\pcolor}} x_{ij}         \label{lpf_2} \\
    
    \forall \pcolor \in \Colors, \forall i \in S: 
    \sum_{j \in \Points^{\pcolor}} x_{ij}       
    \leq  (\alpha_h+\dpc) \Big( \sum_{j \in \Points} x_{ij} \Big)     \label{lpf_3}
    
  \end{align}
\end{subequations}

==> constraint_set_unsquish.tex <==

\begin{subequations}\label{lpf}
  \begin{equation}
    \label{lpf_1}
     \sum_{i,j} d^p(i,j) x_{ij} \leq \upofp
  \end{equation}
  \begin{equation}
    \label{lpf_11}
    \forall j \in \Points: \sum_{i \in S} x_{ij}=1, \quad x_{ij} \in [0,1]
  \end{equation}
  \begin{equation}
    \label{lpf_dpc_orig}
    \forall h \in \Colors: \dpc \in [0,1]
  \end{equation}
    \begin{equation}
    \label{lpf_2}
    \forall \pcolor \in \Colors, \forall i \in S: 
    (\beta_h-\dpc) \Big( \sum_{j \in \Points} x_{ij} \Big) 
    \leq \sum_{j \in \Points^{\pcolor}} x_{ij}       
  \end{equation}
  \begin{equation}
    \label{lpf_3}
    \forall \pcolor \in \Colors, \forall i \in S: 
    \sum_{j \in \Points^{\pcolor}} x_{ij}       
    \leq  (\alpha_h+\dpc) \Big( \sum_{j \in \Points} x_{ij} \Big) 
  \end{equation}
\end{subequations}
